Real-Gas Effects and Phase Separation in Underexpanded Jets at Engine-Relevant Conditions

A numerical framework implemented in the open-source tool OpenFOAM is presented in this work combining a hybrid, pressure-based solver with a vapor-liquid equilibrium model based on the cubic equation of state. This framework is used in the present work to investigate underexpanded jets at engine-relevant conditions where real-gas effects and mixture induced phase separation are probable to occur. A thorough validation and discussion of the applied vapor-liquid equilibrium model is conducted by means of general thermodynamic relations and measurement data available in the literature. Engine-relevant simulation cases for two different fuels were defined. Analyses of the flow field show that the used fuel has a first order effect on the occurrence of phase separation. In the case of phase separation two different effects could be revealed causing the single-phase instability, namely the strong expansion and the mixing of the fuel with the chamber gas. A comparison of single-phase and two-phase jets disclosed that the phase separation leads to a completely different penetration depth in contrast to single-phase injection and therefore commonly used analytical approaches fail to predict the penetration depth.

==> chapter_results_old.tex <==
%!TEX root = main.tex

\section{Results}

The discussion of the results is divided into two parts. First, a single test case is analyzed and defined as the reference case, namely CNG-p600. A special focus will be on the temporal evolution of the near-nozzle flow structure, the evolving two-phase regions and the interactions between the single-phase and two-phase states. In the second part of the discussion the remaining test cases are compared a) to the reference case CNG-p600 and b) against each other (pressure-change, fuel-change).

\subsection{Detailed discussion: CNG-p600}

Fig.~\ref{fig:CNGp600_temporalEvolution} shows snapshots of the temporal evolution of the high-pressure injection of CNG with a total pressure of \SI{600}{\bar} and a total temperature of \SI{300}{\kelvin} into the pressurized mixing chamber ($p_{ch}=\SI{50}{\bar}, T_{ch}=\SI{300}{\kelvin}$) filled with nitrogen at rest (CNG-p600). The left column represents the temperature distribution superimposed by the vapor mass fraction $\beta$. In the right column the pressure field is overlapped by the Mach number, in which regions with $Ma<1$ are excluded. Right at the injection-beginning at \SI{5}{\micro\second} the fluid enters the mixing chamber and a Prandtl-Mayer expansion fan is formed at the nozzle edge. The flow accelerates across the expansion fan, the Mach number increases while the static pressure and temperature drops. The decrease in pressure and temperature and the already premixed fuel leads to a first evolving two-phase region very close to the nozzle trailing edge. The expansion fan interacts with the free jet boundary leading to weak compression waves and an intercepting shock, which distinguishes the jet from the surrounding chamber medium nitrogen. Due to the sharp jet boundary there is almost no mixing present. The traveling spherical vortex breaks open and gets pushed into the mixing chamber by the following steady-state jet region. The intercepting shock ends in a strong curved shock, the Mach disk. At \SI{20}{\micro\second} onwards a small region within the jet core is visible, showing no vapor mass fraction $\beta$ (red circle). After the oblique/normal shock the flow is decelerated and the static pressures and temperatures increase. This rising is enough for the fluid to exit the two-phase region and a single-phase state is approached again. For large pressure ratios resulting in highly underexpanded jets the flow accelerates quickly and reaches a supersonic state with $Ma\gg1$ again. In this supersonic state the velocity increases like before, the pressure and temperature decreases and a two-phase region is formed once more. The first shock barrel ends therefore between the first two two-phase regions inside the jet core. In the snapshots for the times \SI{40}{}, \SI{60}{} and \SI{80}{\micro\second} the initial break-up of the spherical vertex can be traced quite nicely. Beginning at \SI{40}{\micro\second}, a cone is formed in front of the jet which prevents its further penetration into the mixing chamber along the centerline. As a result the fluid gets pushed to the outer regions and the vertex breaks up. Although the flow is detached from the centerline, the static pressures and temperatures remain that low that the initial two-phase region persists. The last frame at the bottom shows the near-nozzle flow structure of the quasi-stationary jet after an injection time of \SI{250}{\micro\second} as all of the mentioned flow properties are only fluctuating around their mean values. A total of four shock barrels and two-phase regions are present in the examined window of Fig.~\ref{fig:CNGp600_temporalEvolution} up to $x/D=\SI{15}{}$.

\begin{figure}[t]
	\centering
	\includetikz{CNGp600_temporalEvolution}
	\caption{Snapshots of the temporal evolution of the evolving two-phase regions for CNG ($p_{t,fuel}=\SI{600}{\bar}$).}
	\label{fig:CNGp600_temporalEvolution}
\end{figure}

A more detailed view of the trailing vertex (marked red rectangle in Fig.~\ref{fig:CNGp600_temporalEvolution}) is visualized in Fig.~\ref{fig:CNGp600_snaps} showing pressure $p$, temperature $T$, methane mass fraction $w_{CH_4}$, speed of sound $a_s$, Mach number $Ma$, isenthalpic compressibility $\psi_h$ and vapor mass fraction $\beta$. Beginning on the left the minimum pressure of the first expansion wave is \SI{8}{\bar} while the compression process in front of the vertex increases the fluid-pressure up to \SI{80}{\bar}. Due to the expansion and compression the temperature ranges from \SI{150}{\kelvin} to \SI{350}{\kelvin} (second frame). The decrease of the premixed CNG (Tab.~\ref{tab:CNGmixture}) leads to an evolving two-phase region mainly in the shock barrel and in a small region above where the appropriate conditions occur. As discussed earlier the speed of sound and the isenthalpic compressibility change significantly due to the liquid mass fraction, resulting in great discontinuities in their respective flow properties. Moreover the speed of sound drops and the Mach number defined as $Ma=u/a_s$ jumps to values up to \SI{4}{}. To the authors knowledge it is the first time that such discontinuities due to the expansion and mixing processes and therefore evolving two-phase regions are shown and presented in CFD simulations in such detail.

\begin{figure}[t]
	\centering
	\includetikz{CNGp600_snaps}
	\caption{Detailed view of different flow properties for CNG-p600.}
	\label{fig:CNGp600_snaps}
\end{figure}

\subsection{Comparison of remaining test cases}

Comparing the near-nozzle flow structure of the direct injection of CNG for both fuel pressures \SI{600}{\bar} and \SI{300}{\bar} in Fig.~\ref{fig:CNG_comparison} a weaker expansion due to the lower pressure ratio of $\Pi=\SI{6}{}$ can be seen. But still the pressures and temperatures are decreased such that a transition of the single-phase to the two-phase state takes place. In contrast to very low vapor mass fractions of \SI{0.5}{} for the high pressure injection indicating a more liquid like state, the vapor mass fractions for the low pressure injection ranging from \SIrange{0.7}{1.0}{} are greater. In addition it can be stated that the break up of the spherical vertex takes place but, in contrast to the high pressure jet, is weakened in its intensity. The last frame indicates a wider spreading angle of the break up in the upper half than in the lower half. Due to the lower fuel pressure and therefore a lower density and speed of sound the penetration of the jet is slower. The stationary shock barrels are smaller in their length by a factor of almost two, correlating with the predictions of Velikorody and Kudriakov~\cite{velikorodny2012numerical}.

\begin{figure}[t]
	\centering
	\includetikz{CNG_comparison}
	\caption{Comparison of the near-nozzle flow structure by lowering the fuel pressure from \SI{600}{\bar} (upper half) to \SI{300}{\bar} (lower half) for CNG.}
	\label{fig:CNG_comparison}
\end{figure}

Fig.~\ref{fig:CNGCHG300_comparison} shows the effects of the fuel change from CNG to CHG for a total pressure of \SI{300}{\bar}. For each fluid the temperature is plotted. In case of the CNG-jet the temperature is superimposed by the vapor mass fraction $\beta$. Although the expansion of CHG is much stronger with temperatures down to \SI{100}{\kelvin} compared to CNG with temperatures down to \SI{150}{\kelvin}, the fluid remains in a single-phase state. This is mainly due to the composition of CHG, containing \SI{99.9}{vol\percent} hydrogen with a critical temperature of $T_c=\SI{33.15}{\kelvin}$ and \SI{0.1}{vol\percent} nitrogen with $T_c=\SI{126.19}{\kelvin}$. The volume fraction of nitrogen in the premixed fuel does not suffice to increase the critical temperature of the mixture such that it is higher than the minimum temperature in the core of the jet. Thus no transition from the single-phase state to a two-phase state takes place. The opening jet angle for CHG is greater and the length of the shock barrel smaller. For the CHG-p600-case, which neither shows any evolved two-phase regions, the same conclusions can be drawn.

\begin{figure}[t]
	\centering
	\includetikz{CNGCHG300_comparison}
	\caption{Comparison of the near-nozzle flow structure for CNG (upper half) and CHG (lower half) and a fuel pressure of \SI{300}{\bar}.}
	\label{fig:CNGCHG300_comparison}
\end{figure}

Using the one-dimensional flow analysis presented in Banholzer~et~al.~\cite{banholzer2017} the choked flow properties of the two fuels for the different operating conditions can be calculated (see Tab.~\ref{tab:critNozzle}) and some of the effects due to fluid and pressure change discussed earlier are explicable. A first mention should be made of the fact that CHG chokes much earlier at pressures of \SI{279.62}{\bar} and \SI{148.09}{\bar}, while the critical pressure $p^\ast$ of CNG is significantly lower at \SI{191.37}{\bar} and \SI{124.66}{\bar}. In our case the back/chamber pressure is \SI{50}{bar} and therefore importantly lower than the choked flow pressures in Tab.~\ref{tab:critNozzle}. As a result the flow is choked for all four test scenarios. For this type of flow the maximum mass flow through the orifice can be evaluated as $\dot{m}_n^\ast = \rho^\ast a_s^\ast A$ with $A$ being the cross-sectional area of the nozzle. Flow losses due to detachments caused by the shape of the nozzle (among other things) can decrease the mass flow by up to \SI{20}{\percent}~\cite{tang1978experimental}. The reduction of the achievable mass flow is known as discharge coefficient and is defined as $C_d = \dot{m} / \dot{m}_n^\ast$. For the lower fuel pressure of \SI{300}{\bar} the maximum mass flow of CNG is \SI{115.59}{\gram\per\second} and therefore $3.6$-times higher than for CHG (\SI{32.09}{\gram\per\second}), mainly due to the much higher density of $\rho^\ast = \SI{148.87}{\kilogram\per\meter\cubed}$ compared to \SI{13.65}{\kilogram\per\meter\cubed} for CHG, although the speed of sound is much higher for CHG. Doubling the pressure to \SI{600}{\bar} results in a maximum mass flow of \SI{62.02}{\gram\per\second} for CHG (an increase of \SI{93.3}{\percent}) in contrary to \SI{216.86}{\gram\per\second} for CNG (an increase of \SI{87.6}{\percent}).

Discussing the penetration depth of the jet the main influencing parameter is the momentum flux provided at the nozzle exit~\cite{abraham1996entrapment,hill1999transient,gerold2013new} which is defined as $\dot{M}_n^\ast = \rho^\ast {a_s^\ast}^2 A$. For the lower fuel pressure of \SI{300}{\bar} the value evaluated for the CNG-case is \SI{50.78}{\kilogram\meter\per\second\squared} and therefore \SI{19.0}{\percent} higher than for CHG (\SI{42.68}{\kilogram\meter\per\second\squared}). The difference of the two fluids is not as great as before when discussing the mass flux as the momentum flux is proportional to the squared speed of sound. For a fuel pressure of \SI{600}{\bar} the momentum flux for CNG increases by \SI{137.6}{\percent} to \SI{120.67}{\kilogram\meter\per\second\squared} while for CHG the momentum flux increases by \SI{113.5}{\percent} to \SI{91.11}{\kilogram\meter\per\second\squared}. Comparing the values for both fuels and operating points it is presumed that the CNG-jet with \SI{600}{\bar} penetrates the fastest, followed by CHG-p600, CNG-p300 and CHG-p300.

\begin{table}[!htb]
%	\vspace{-12pt}
	\centering
	\caption{Choked nozzle flow properties for CHG and CNG ($T_{t,fuel}=\SI{300}{\kelvin}$, SRK-EoS).}
%	\vspace{6pt}
	\begin{tabular}{c|c|ccccc}
		\toprule
		\multirow{ 2}{*}{Fuel}  & $p_{t,fuel}$ & $p^\ast$ & $\rho^\ast$ & $a_s^\ast$ & $\dot{m}_n^\ast$ & $\dot{M}_n^\ast$ \\
								& [\si{bar}] & [\si{bar}] 	& [\si{\kilogram\per\meter\cubed}] 	& [\si{\meter\per\second}] 	  & [\si{\gram\per\second}] 	  & [\si{\kilogram\meter\per\second\squared}] \\
		\midrule
		\multirow{ 2}{*}{CNG}	& 600 & 191.37 & 220.55 & 556.42 & 216.86 & 120.67 \\
		    					& 300 & 124.66 & 148.87 & 439.36 & 115.59 & 50.78 \\
		\midrule
		\multirow{ 2}{*}{CHG}   & 600 & 279.61 & 23.87 & 1469.18 & 62.02 & 91.11 \\
			 					& 300 & 148.09 & 13.65 & 1330.11 & 32.09 & 42.68 \\
		\bottomrule 
	\end{tabular}
	\label{tab:critNozzle}
%	\vspace{-12pt}
\end{table}

Performing simulations of high-pressure injections with the above mentioned operating points is a very challenging task in terms of physical modeling (e.g. consistent thermodynamics), numerical schemes (e.g. shock capturing) and computational power. Due to the latter aspect the near-nozzle flow structure of all four test cases was discussed while the jet penetration depth will only be analyzed for CNG-p300 and CHG-p300. Fig.~\ref{fig:Ztip} shows the normalized jet penetration depths ${Z}_{tip}/D$ resulting from the numerical simulations, captured with a mass fraction of $w_{fuel}=\SI{0.01}{}$ at the centerline, with a detailed view of the injection-beginning on the right. Up to \SI{0.2}{ms} the kinetic momentum flux $J^\ast = {a_s^\ast}^2 A$ is dominant~\cite{abraham1996entrapment} and the CHG-p300-jet penetrates faster than the CNG-p300-jet with the same total pressure. While in the beginning of the injection the penetration curve shows a linear incline due to the detachment of the jet from the centerline, the jet reattaches at around \SI{0.09}{\milli\second} and the penetration profile is in a very good agreement with the correlation of Hill and Ouellette~\cite{hill1999transient} with the fitting parameter of $\Gamma=\SI{2.968}{}$ obtained in Banholzer~et~al.~\cite{banholzer2017}, see dashed lines. A first conclusion can be drawn that although the injection is performed at elevated pressures and therefore real-gas effect need to be modeled, the penetration depth for gas-like, single-phase jets can still be estimated by a rather simple correlation.

\begin{figure}[!htb]
	\centering
	\includetikz{Ztip}
	\caption{Normalized jet penetration depths ${Z}_{tip}/D$ for all test cases.}
	\label{fig:Ztip}
\end{figure}

The results for the injection profile for the CNG-p300-case differ completely. Not only in the beginning, but almost throughout the whole computational domain the linear incline remains. Shortly before \SI{0.5}{\milli\second} it can be seen that the linear incline changes to the typical curvature known for transient gaseous jets and the jet penetration is proportional to the square root of time. The major reason for this extraordinary behavior is the traveling spherical vertex. Fig.~\ref{fig:CNG_comparison} and \ref{fig:CNGCHG300_comparison} show large two-phase regions in the first vertex, which remain present even for longer simulation times. Later, increasing temperatures and pressures lead to the disappearance of those, momentum gets lost and the jet slows down. Comparing the jet penetration depth and the vanishing of the two-phase region the time where the slope changes its characteristic is identical. The same conclusions can be drawn for the \SI{600}{\bar}-cases and are therefore not discussed further.






